An Estimation and Analysis Framework for the Rasch Model

The Rasch model is widely used for item response analysis in applications ranging from recommender systems to psychology, education, and finance. While a number of estimators have been proposed for the Rasch model over the last decades, the available analytical performance guarantees are mostly asymptotic. This paper provides a framework that relies on a novel linear minimum mean-squared error (L-MMSE) estimator which enables an exact, nonasymptotic, and closed-form analysis of the parameter estimation error under the Rasch model. The proposed framework provides guidelines on the number of items and responses required to attain low estimation errors in tests or surveys. We furthermore demonstrate its efficacy on a number of real-world collaborative filtering datasets, which reveals that the proposed L-MMSE estimator performs on par with state-of-the-art nonlinear estimators in terms of predictive performance.

==> 1-introduction.tex <==
% !TEX root = 18ICML_linrasch.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Introduction}
%
This paper deals with the estimation of the $N$-dimensional vector $\bmx\in\reals^N$ from the \emph{probit model} \cite{firstprobit}
\begin{align} \label{eq:probitmodel}
\bmy = \sign(\bD\bmx+\bmw).
\end{align}
Here, the vector $\bmy\in\{-1,+1\}^M$ contains $M$ binary-valued measurements, the  function $\sign(z)$ operates element-wise on its argument and outputs $+1$ for $z\geq0$ and $-1$ otherwise, $\bD\in\reals^{M\times N}$ is a given design matrix (or matrix of covariates), and the vector $\bmw\in\reals^M$ has i.i.d.\ standard normal entries.  
%
Estimation of the vector $\bmx$ from the observation model in \fref{eq:probitmodel} is known as \emph{probit regression}, which finds widespread use---along with related methods, such as logistic regression  \cite{logregfirst}---in a broad range of applications and fields, including (but not limited to) image classification~\cite{imageclassification}, biomedical data analysis~\cite{cancer,biology}, economics~\cite{economy}, educational data mining~\cite{lordirt}, and signal processing~\cite{larry,plan1bit}. 

\subsection{Relevant Prior Art}
%
\paragraph{Estimators}
%
The two most common estimation techniques for the probit model in~\fref{eq:probitmodel} are the posterior mean (PM) and maximum a-posteriori (MAP) estimators. 
%
The PM estimator computes the following conditional expectation \cite{poorbook}:
\begin{align} \label{eq:PME}
\hat\bmx^\text{PM} =\textstyle  \Ex{\bmx}{\bmx| \bmy} = \int_{\reals^N} \bmx p(\bmx|\bmy)\text{d}\bmx,
\end{align}
where $p(\bmx|\bmy)$ is the posterior probability of the vector $\bmx$ given the observations $\bmy$ under the model  \fref{eq:probitmodel}. The PM estimator is optimal in a sense that it minimizes the mean-squared error (MSE) defined as
\begin{align} \label{eq:MSE}
\textit{MSE}(\hat\bmx) = \Ex{\bmx,\bmw}{\|\bmx-\hat\bmx\|^2},
\end{align} 
and is, hence, also known as the nonlinear minimum mean-squared error (MMSE) estimator. Evaluating the integral in~\fref{eq:PME} for the probit model is difficult and hence, one typically resorts to rather slow Monte-Carlo methods \cite{albertchib}. 
%
By assuming that the vector $\bmx$ is multivariate Gaussian, an alternative regression technique is the MAP estimator that solves the following convex optimization problem~\cite{probitml}:
\begin{align} \label{eq:MAPestimator}
\hat\bmx^\text{MAP} = \textstyle \underset{\bmx\in\reals^N}{\text{arg\,min}}   -\!\sum_{m=1}^M \log(\Phi(y_m \bmd_m^T \bmx)) + \frac{1}{2} \bmx^T \bC_{\bmx}^{-1} \bmx.
\end{align}
Here, $\Phi(x)=\int_{-\infty}^x (2\pi)^{-1/2}e^{-t^2/2}\text{d}t$ is the cumulative distribution function of a standard normal random variable, $\bmd^T_m$ is the $m$th row of the covariate matrix $\bD$, and $\bC_\bmx$ is the covariance matrix of the zero-mean multivariate Gaussian prior on the vector~$\bmx$. By ignoring the prior on $\bmx$, one arrives at the well-known maximum-likelihood (ML) estimator. 
%
Compared to the PM estimator, MAP and ML estimation can be implemented more efficiently by solving a series of re-weighted least squares problems \cite{tibsbook} or simply by using standard numerical methods for convex problems that scale favorably to large problem sizes \cite{wrightbook}. 
%
In contrast to such well-established, nonlinear estimators, we will investigate \emph{linear estimators} that are computationally efficient and show that their performance is on par to that of the PM, MAP, and ML estimators. 

\paragraph{Analytical Results}
%
Analytical results that characterize the performance of estimation under the probit model are almost exclusively for the \emph{asymptotic} setting.  
%
More specifically, Brillinger  \cite{brillinger1982generalized} has shown in 1982 that the use of conventional least-squares (LS) estimators for scenarios in which the design matrix $\bD$ has i.i.d.\ Gaussian entries, deliver an estimate that is the same as that of the PME up to a constant. 
%
More recently, Brillinger's result has been generalized by Thrampoulidis \emph{et al.}~\cite{thrampoulidis2015lasso} to the sparse setting, i.e., where the vector~$\bmx$ has only a few nonzero entries. 
%
Another strain of results focuses on a performance analysis of ML estimators using the asymptotic normality property~\cite{mlasymptotoicglm,mlasymptoticlogit}.  These results provide \emph{lower bounds} on the MSE using the Fisher information matrix \cite{datasetbook} as the number $M$ of measurements goes to infinity.  
%
Some recent results analyze the consistency of the ML estimator for sparse logistic regression.  
%
These results are either asymptotic \cite{honestlogit,plan1bit,wainwrightising} or of probabilistic nature \cite{bachlogit}; the latter kind bounds the MSE with high probability. 
%%
In contrast to all such existing analytical results, we will provide \emph{nonasymptotic} and \emph{exact} expressions for the MSE that are valid for \emph{arbitrary} and \emph{deterministic} design matrices $\bD$. 


\subsection{Contributions}
%
We propose to (i) design novel \emph{linear estimators} of the form $\hat\bmx=\bW\bmy$ for the probit model in \fref{eq:probitmodel}, where $\bW\in\reals^{N\times M}$ are suitably-chosen estimation matrices, and (ii) provide \emph{exact}, \emph{closed-form}, and \emph{nonasymptotic} expressions for the MSE of these estimators.  
%
Specifically, we will develop two estimators: a linear minimum mean-squared error (L-MMSE) estimator that aims at minimizing the MSE in \fref{eq:MSE}  and a more efficient but less accurate least-squares~(LS) estimator.
%
Our MSE results are in stark contrast to existing performance guarantees for the MAP or PM estimators, for which a nonasymptotic performance analysis is, in general, difficult.  
%
To demonstrate the efficacy of our analysis, we derive exact MSE performance results for the Rasch model \cite{rasch}, which is widely used in psychometrics, e.g.,  for the analysis of user responses to test items. 
%
We  provide inference results on synthetic data, which suggest that the inference quality of the proposed linear estimators is on par with state-of-the-art nonlinear estimators, especially at low signal-to-noise ratio (SNR), when the quantization error level is lower than the noise level.  Moreover, we show using ten different real-world regression and collaborative filtering datasets that the proposed linear estimators achieve competitive predictive performance to PM and MAP estimation and at comparable or even lower complexity.




==> 2-mainresults.tex <==
% !TEX root = 18ICML_linrasch.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Linearized Probit Regression}
\label{sec:mainresults}

To develop and analyze linearized inference methods for the standard probit model in \fref{eq:probitmodel}, we will consider the following (slightly) generalized version of the probit model:
\begin{align} \label{eq:probitmodelgeneral}
\bmy = f_\sigma(\bD\bmx+\bmw).
\end{align} 
Here, $\bmy\in[-1,+1]^M$, $\bmx$ is zero-mean Gaussian with known covariance~$\bC_\bmx$, the sigmoid function is defined as 
$f_\sigma(z) = 2 \Phi(z/\sigma) - 1$ and operates element-wise on its argument, $\sigma\in(0,\infty)$ is a smoothing parameter, and the vector $\bmw$ is assumed to be zero-mean Gaussian with known covariance~$\bC_\bmw$ and independent of $\bmx$.\footnote{We emphasize that these are standard model assumptions in Bayesian data analysis (see, e.g., \cite{hoffbook}) and in numerous real-world applications, such as modeling user responses to test items \cite{lordirt}.}
%%
In what follows, we assume nondegenerate covariance matrices for $\bmx$ and $\bmw$, i.e., we assume that~$\bC_{\bmx}$ and $\bC_\bmw$ are both invertible. 
%
We emphasize that as $\sigma\to0$, the sigmoid function $f_\sigma(z)$ corresponds to the sign function and hence, the model in \fref{eq:probitmodelgeneral} includes the probit model in \fref{eq:probitmodel} as a special case. 
%
We next introduce two new linear estimators for this model and then, provide exact, closed-form, and nonasymptotic expressions for their associated MSEs.


\subsection{Linear Minimum Mean-Square Error Estimator}
%

%
Our main  result is as follows.
%
\begin{thm} \label{thm:lmmseestimator}
%
The linear minimum mean-square error (L-MMSE) estimate for the generalized probit model in \fref{eq:probitmodelgeneral} is
\begin{align} \label{eq:LMMSE}
\hat\bmx^\text{\em L-MMSE} = \bE^T \bC_\bmy^{-1}\bmy,
\end{align}
where
\begin{align} 
%\bE = \textstyle \sqrt{\frac{2}{\pi}} \mathrm{diag}(\mathrm{diag}(\bC_\bmz))^{-1/2})\bD\bC_\bmx,
\bE & =  \textstyle \left(\frac{2}{\pi}\right)^{1/2} \mathrm{diag}(\mathrm{diag}(\sigma^2\bI+\bC_\bmz)^{-1/2})\bD\bC_\bmx,\label{eq:Ematrixcompact} \\
\notag \bC_\bmy & =\textstyle  \frac{2}{\pi} \arcsin ( \mathrm{diag}( \mathrm{diag}(\sigma^2\bI+\bC_\bmz)^{-1/2})  \bC_\bmz \\ & \quad \quad \times \mathrm{diag}(\mathrm{diag}(\sigma^2\bI+\bC_\bmz)^{-1/2}) ), \label{eq:arcsinelawcompact}
\end{align}
and $\bC_\bmz=\bD\bC_\bmx\bD^T+\bC_\bmw$.
%
\end{thm}






\begin{proof}
%
The proof consists of two steps. First, we linearize the model in \fref{eq:probitmodelgeneral}.
%
Then, we derive the L-MMSE estimate in~\fref{eq:LMMSE} for the linearized model. The two  steps are as follows. 

%%%
{\em Step 1 (Linearization): } Let $\bmz=\bD\bmx+\bmw$ and 
\begin{align} \label{eq:bussgang}
\bmy=f_\sigma(\bmz)=\bF\bmx+\bme
\end{align} be a linearization of the generalized probit model in \fref{eq:probitmodelgeneral}, where $\bF\in\reals^{M\times N}$  is a \emph{linearization matrix} and $\bme\in\reals^M$ is a \emph{residual error vector} that contains noise and linearization artifacts. 
%
Our goal is to perform a Bussgang-like decomposition \cite{bussgang}, which uses the linearization matrix~$\bF$ that minimizes the $\ell_2$-norm of the residual error vector~$\bme$ averaged over the signal and noise.
%
Concretely, let~$\bC_\bmz$ be the covariance matrix of the vector $\bmz$ and consider the optimization problem
\begin{align*}
\underset{\bF\in\reals^{M\times N}}{\mathrm{minimize}} \; \Ex{\bmx,\bmw}{\big\|\bmy - \bF\bmx\big\|^2}\!,
\end{align*}
which has a closed-form solution that is given by $\bF = \bE \bC^{-1}_\bmx$ with $\bE= \Ex{\bmx,\bmw}{\bmy\bmx^T}$.
%
It can easily be verified that for this particular choice of the linearization matrix $\bF$, the residual error vector $\bme$ and the signal of interest $\bmx$ are uncorrelated, i.e., we have $\Ex{\bmx,\bmw}{\bmx\bme^T}=\bZero_{N\times M}$.


We now derive a closed-form expression for the entries of the matrix $\bE$.  Since both $\bmx$ and $\bmw$ are independent and zero-mean Gaussian, the bivariate $(z_m,x_n)$ is jointly Gaussian for each index pair $\{m,n\}$. Moreover, we have $\Ex{t}{\abs{f_\sigma(t)}} < \infty$ and $\Ex{t}{\abs{t f_\sigma(t)}} < \infty$ if~$t$ is a zero-mean Gaussian random variable. Hence, we can use the following result that is due to Brillinger \citep[Lem.~1]{brillinger}:
\begin{align} \label{eq:brillinger}
[\bE]_{m,n}  = \Ex{\bmx,\bmw}{y_mx_n} = \frac{\textit{Cov}(z_m,x_n)}{\textit{Var}(z_m)} \Ex{z_m}{y_mz_m}\!,
\end{align}
where $\textit{Cov}(z_m,x_n)= \bmd_m^T\bmc_n$ with $\bmc_n$ being the $n$th column of $\bC_\bmx$.
%
Since for $\sigma>0$ the function $y_m= f_\sigma(z_m)$ is absolutely continuous\footnote{The special case for $f_0(z_m)$ can either be derived by directly evaluating $\Ex{}{\sign(z_m)z_m}$ in \fref{eq:brillinger} or by first using Stein's Lemma and then letting $\sigma\to0$; both approaches yield the same result.}, $z_m$ is zero-mean Gaussian, and $\Ex{t}{f'_\sigma(t)} < \infty$,  we can invoke Stein's Lemma~\cite{stein}, which states that
\begin{align} \label{eq:stein}
\frac{\Ex{z_m}{f_\sigma(z_m)z_m}}{\textit{Var}(z_m)} = \Ex{z_m}{f'_\sigma(z_m)}
\end{align}
with $f'_\sigma(z)=\frac{\text{d}}{\text{d}z} f_\sigma(z)$.
%
Using $f_\sigma(x) = 2 \Phi(x/\sigma) - 1$, we can evaluate the right-hand side in \fref{eq:stein} as 
%
\begin{align}
 \Ex{z_m}{f'_\sigma(z_m)} & \textstyle = 2 \Ex{z_m}{ \Phi'\!\left({z_m}/{\sigma}\right)} \notag \\
& = \textstyle \frac{2}{\sigma} \int_{-\infty}^\infty \mathcal{N} \!\left({z_m}/{\sigma}; 0,1\right) \mathcal{N} (z_m; 0, \gamma_m) \mathrm{d} z_m  \notag \\
%
& \textstyle = \frac{2}{\sigma} \frac{\sigma'}{\sqrt{2 \pi\gamma_m}}  \int_{-\infty}^\infty \frac{1}{\sqrt{2 \pi} \sigma'} \exp\!\left(-\frac{z_m^2}{2 \sigma'^2}\right)\! \mathrm{d} z_m \notag \\
%& =  \frac{2}{\sigma} \frac{1}{\sqrt{2 \pi} \sqrt{\gamma_m}} \frac{\sigma \sqrt{\gamma_m}}{\sqrt{\sigma^2 + \gamma_m}} \\
& = \textstyle \left(\frac{2}{\pi}\right)^{1/2}\! \frac{1}{\sqrt{\sigma^2 + \gamma_m}}, \label{eq:laststep1}
%& = \sqrt{\frac{2}{\pi}} \frac{1}{\sqrt{\gamma_m}} \\
\end{align}
where  $\mathcal{N} (z; \mu, \sigma^2)$ denotes the probability density function of a Gaussian distribution with mean $\mu$ and variance $\sigma^2$ evaluated at $z$, $\gamma_m=\textit{Var}(z_m) = \bmd_m^T \bC_\bmx \bmd_m + [\bC_\bmw]_{m,m}$, and $\sigma'^2 = \frac{\sigma^2 \gamma_m}{\sigma^2 + \gamma_m}$.
%
Combining \fref{eq:brillinger} with \fref{eq:stein} and \fref{eq:laststep1} leads to 
%
\begin{align*}
[\bE]_{m,n} \textstyle = \left(\frac{2}{\pi}\right)^{1/2}\! \frac{ \bmd_m^T\bmc_n}{\sqrt{\sigma^2 + \bmd_m^T \bC_\bmx \bmd_m + [\bC_\bmw]_{m,m}}},
\end{align*}
where \fref{eq:Ematrixcompact} represents the entire matrix $\bE$ in compact notation.





%%%
{\em Step 2 (L-MMSE Estimator): }
%
We have linearized the probit model as $\bmy=f_\sigma(\bmz)=\bF\bmx+\bme$ in~\fref{eq:bussgang} with $\bF = \bE \bC^{-1}_\bmx$. We now estimate $\bmx$ from this linearization using the L-MMSE estimator.
%
Since the residual distortion vector $\bme$ is uncorrelated to the vector $\bmx$, the L-MMSE estimator is given by  
\begin{align*}
\hat\bmx^\text{L-MMSE} = \bE^T \bC_\bmy^{-1}\bmy,
\end{align*}
where $\bC_\bmy=\Ex{\bmx,\bmw}{\bmy\bmy^T}$ is the covariance matrix of the generalized probit measurements in \fref{eq:probitmodelgeneral}.
%
The remaining piece is to calculate the individual entries of this matrix. 

With abuse of notation, we start by deriving the necessary expressions for a general pair of correlated but zero-mean Gaussian random variables $(x,y)$ with covariance matrix $\bC = [C_{x,x},C_{x,y};  C_{x,y} ,C_{y,y}]$.
%
More specifically, we are interested in computing the quantity 
\begin{align*}
\Ex{x,y}{f_\sigma(x)f_\sigma(y)} 
%&= \Ex{x,y}{(2\Phi({x}/{\sigma})-1) (2\Phi({y}/{\sigma})-1)} \\
& = 4 \Ex{x,y}{\Phi({x}/{\sigma}) \Phi({y}/{\sigma})} + 1 \\
& \quad - 2\Ex{x}{\Phi({x}/{\sigma})} - 2\Ex{y}{\Phi({y}/{\sigma})} .
%& = \frac{2}{\pi} \arcsin \frac{C_{x,y}}{\sqrt{\sigma^2 + C_{x,x}} \sqrt{\sigma^2 + C_{y,y}}},
\end{align*}
Since
\begin{align*}
& \Ex{x}{\Phi({x}/{\sigma})} = \textstyle \int_{-\infty}^\infty \Phi({x}/{\sigma}) \mathcal{N}(x; 0, C_{x,x}) \mathrm{d} x  \\
%& = \int_{-\infty}^0 \Phi({x}/{\sigma}) \mathcal{N}(x; 0, C_{x,x}) \mathrm{d} x + \int_0^\infty \Phi({x}/{\sigma}) \mathcal{N}(x; 0, C_{x,x}) \mathrm{d} x \\
 & \quad = \textstyle \int_0^\infty (\Phi(-{x}/{\sigma}) + \Phi({x}/{\sigma}))  \mathcal{N}(x; 0, C_{x,x}) \mathrm{d} x 
% & = \int_0^\infty \mathcal{N}(x; 0, C_{x,x}) \mathrm{d} x 
 = \frac{1}{2},
\end{align*}
we have
\begin{align} \label{eq:momentsrelation}
\Ex{x,y}{f_\sigma(x)f_\sigma(y)} &= 4 \Ex{x,y}{\Phi({x}/{\sigma}) \Phi({y}/{\sigma})} -1.
\end{align}
%
Hence, we only need a closed-form expression for $\Ex{x,y}{\Phi({x}/{\sigma}) \Phi({y}/{\sigma})}$, which we derive using direct integration. 
%
We rewrite this expression as follows:
\begin{align*}
& \Ex{x,y}{\Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{y}{\sigma}\right)} 
= \int_{-\infty}^\infty \int_{-\infty}^\infty \Phi\!\left(\frac{x}{\sigma}\right) \Phi\!\left(\frac{y}{\sigma}\right) \\ 
& \quad \times \mathcal{N} \!\left( \left[ \begin{array}{c} x \\ y \end{array} \right]; \bm0, \left[ \begin{array}{cc} C_{x,x} & C_{x,y} \\ C_{x,y} & C_{y,y} \end{array} \right] \right)\! \mathrm{d}x \mathrm{d}y \\
%= & \int_{-\infty}^\infty \Phi({x}/{\sigma}) \left( \int_{-\infty}^\infty \Phi({y}/{\sigma}) \mathcal{N}\!\left(\!y; \frac{C_{x,y}}{C_{x,x}}, C_{y,y} - \frac{C_{x,y}^2}{C_{x,x}}\right)\! \mathrm{d}y \!\right)\! \mathcal{N}(x; 0, C_{x,x}) \mathrm{d}x \\
& \quad = \int_{-\infty}^\infty \Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{x}{\sigma'}\right) \mathcal{N}(x; 0, C_{x,x}) \mathrm{d}x,
\end{align*}
where the last equality follows from \citep[Sec.~3.9]{gpml} with $\sigma' = \frac{C_{x,x}}{C_{x,y}} \sqrt{\sigma^2 + C_{y,y} + \frac{C_{x,y}^2}{C_{x,x}}}$.  We now further simplify the above expression with the following steps:
\begin{align*}
& \Ex{x,y}{\Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{y}{\sigma}\right)} \\
& \quad = \int_{-\infty}^\infty \Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{x}{\sigma'}\right)\! \frac{1}{\sqrt{2 \pi C_{x,x}}} \exp\!\left(-\frac{x^2}{2 C_{x,x}}\right)\! \mathrm{d}x \\
%= & \int_{-\infty}^\infty  \Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{y}{\sigma'}\right)\! \frac{1}{\sqrt{2 \pi}} \exp\!\left(-\frac{x^2}{2 C_{x,x}}\right)\! \mathrm{d} \frac{x}{\sqrt{C_{x,x}}} \\
&  \quad =  \int_{-\infty}^\infty \Phi\bigg(\frac{\sqrt{C_{x,x}}}{\sigma}x\bigg) \Phi\bigg(\frac{\sqrt{C_{x,x}}}{\sigma'}x\bigg) \mathcal{N}(x; 0,1) \mathrm{d} x.
\end{align*}
Using the definitions $\sigma_1 = {\sigma}/\!{\sqrt{C_{x,x}}}$ and $\sigma_2= {\sigma'}/\!{\sqrt{C_{x,x}}}$, we can rewrite the above expression as
\begin{align*}
& \Ex{x,y}{\Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{y}{\sigma}\right)} = \int_{-\infty}^\infty \int_{-\infty}^{\frac{x}{\sigma_1}} \int_{-\infty}^{\frac{x}{\sigma_2}} \\
& \quad \quad \qquad \mathcal{N}(y; 0,1)  \mathcal{N}(z; 0,1) \mathrm{d} z \mathrm{d} y\, \mathcal{N}(x; 0,1) \mathrm{d} x.
\end{align*}
%
To evaluate this expression, it is key to observe that this is a cumulative probability density of a 3-dimensional normal random variable with zero mean and an identity covariance matrix on a region cut by two planes.  Imagine a cuboid with edge lengths $\{1, {1}/{\sigma_1}, {1}/{\sigma_2}\}$.  Assume $C_{x,y} > 0$ without loss of generality. The first plane has the normal vector $[1, -\sigma_1, 0]^T$, while the second plane has the normal vector $[1, 0, -\sigma_2]^T$. 
%
To find a convenient way to evaluate this integral, we need to find an appropriate change of coordinates.  Define the first new coordinate $x'$ as the intersection of the two planes, along the direction of $[1, {1}/{\sigma_1}, {1}/{\sigma_2}]^T$.  With proper normalization, this implies $x' = \frac{\sigma_1 \sigma_2 x + \sigma_2 y + \sigma_1 z}{\sqrt{\sigma_1^2 \sigma_2^2 + \sigma_1^1 + \sigma_2^2}}$.  
Then, we let the second coordinate $y'$ be orthogonal to $x'$ and also to the first plane, i.e., orthogonal to the normal vector of the first plane, $[1, {1}/{\sigma_1}, {1}/{\sigma_2}]^T$.  This gives $y' = \frac{\sigma_1^2 x + \sigma_1 y - \sigma_2 (\sigma_1^2 + 1) z}{\sqrt{\sigma_1^2 + 1}\sqrt{\sigma_1^2 \sigma_2^2 + \sigma_1^1 + \sigma_2^2}}$. 
%
The third coordinate is simply $z' = \frac{x - \sigma_1 y}{\sqrt{\sigma_1^2 + 1}}$, taken as the normal vector to the first plane.  The unit vector in the second plane that is orthogonal to $x'$ and $y'$ is given by $v' = \frac{\sigma_2^2 x - \sigma_1(\sigma_2^2 + 1) y - \sigma_2 z}{\sqrt{\sigma_2^2 + 1}\sqrt{\sigma_1^2 \sigma_2^2 + \sigma_1^1 + \sigma_2^2}}$. With this vector, we see that $v'^T y' = -\frac{1}{\sqrt{\sigma_1^2 + 1} \sqrt{\sigma_2^2 + 1}}$, meaning that the angle between $y'$ and $v'$ is larger than $\frac{\pi}{2}$ if $C_{x,y} > 0$ and smaller than $\frac{\pi}{2}$ if $C_{x,y} < 0$. 

Since the new coordinates form a Cartesian system and are properly normalized, the determinant of the Jacobian is one, and the covariance matrix of the 3-dimensional normal random variable remains an  identity matrix. We first integrate over~$x'$ to obtain
\begin{align*}
\textstyle \Ex{x,y}{\Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{y}{\sigma}\right)} = & \textstyle \int\!\! \int_\mathcal{C} \mathcal{N}(y'; 0,1) \mathcal{N}(z'; 0,1) \mathrm{d} y' \mathrm{d} z' ,
\end{align*}
where we have used $\mathcal{C}$ to denote the space to integrate over for the variables $y'$ and $z'$.  Since $\mathcal{C}$ is the area between the directions of $y'$ and $v'$ in the 2-dimensional plane, we use polar coordinates $y' = \rho \cos\theta$ and $z' = \rho \sin\theta$ to get
\begin{align*} 
& \textstyle \Ex{x,y}{\Phi\!\left(\frac{x}{\sigma}\right)\! \Phi\!\left(\frac{y}{\sigma}\right)} \\
& \,\, =   \textstyle \int_0^{\frac{\pi}{2}+\arcsin\!\left( \frac{1}{\sqrt{\sigma_1^2 + 1} \sqrt{\sigma_2^2 + 1}}\right)} \int_0^\infty \frac{1}{2 \pi} e^{-\frac{\rho^2}{2}} \rho \mathrm{d}\rho \mathrm{d} \theta \\
%\notag = & \frac{1}{2 \pi} \left(\frac{\pi}{2}+\arcsin\!\left(\frac{1}{\sqrt{\sigma_1^2 + 1} \sqrt{\sigma_2^2 + 1}}\right)\right) \\
%& =  \textstyle \frac{1}{4} + \frac{1}{2 \pi} \arcsin\!\left(\frac{1}{\sqrt{\sigma_1^2 + 1} \sqrt{\sigma_2^2 + 1}}\right)  \\
& \,\, = \textstyle  \frac{1}{4} + \frac{1}{2 \pi} \arcsin\!\left(\frac{C_{x,y}}{\sqrt{\sigma^2 + C_{x,x}} \sqrt{\sigma^2 + C_{y,y}}}\right)\!. %\label{eq:Cy}
\end{align*}
Consequently, we have
\begin{align*} 
\Ex{x,y}{f_\sigma(x)f_\sigma(y)} =\textstyle  \frac{2}{\pi} \arcsin\!\left(\frac{C_{x,y}}{\sqrt{\sigma^2 + C_{x,x}} \sqrt{\sigma^2 + C_{y,y}}}\right)\!,
\end{align*}
which allows us, in combination with \fref{eq:momentsrelation},  to express the desired covariance matrix $\bC_\bmy$ as in \fref{eq:arcsinelawcompact}.  
\end{proof}



For the L-MMSE estimator in \fref{thm:lmmseestimator}, we can extract the MSE in closed form:
%
\begin{lem} \label{lem:mseoflmmseestimator}
%
The MSE of the L-MMSE estimator in \fref{thm:lmmseestimator} is given by
\begin{align*}
\textit{MSE}(\hat\bmx^\text{\em L-MMSE}) = \tr(\bC_\bmx - \bE^T \bC_\bmy^{-1} \bE).
\end{align*}
\end{lem}
\begin{proof}
The proof follows from the MSE definition  in \fref{eq:MSE} and the facts that $\bF = \bE \bC^{-1}_\bmx$ and the two vectors $\bmx$ and $\bme$ are uncorrelated for the L-MMSE estimator in \fref{eq:LMMSE}.
\end{proof}
%
 







As an immediate consequence of the fact that the PM estimator minimizes the MSE,  we can use \fref{lem:mseoflmmseestimator} to obtain the following upper bound on the MSE of the PM estimator:
\begin{align} \label{eq:PMbound}
\textit{MSE}(\bmx^\text{PM}) \leq \tr(\bC_\bmx - \bE^T \bC_\bmy^{-1} \bE).
\end{align}
As it will be shown in the experiments section, this upper bound on the MSE is surprisingly tight in most situations.


By letting the parameter $\sigma\to0$ in \fref{eq:probitmodelgeneral}, we can use \fref{thm:lmmseestimator} and 
\fref{lem:mseoflmmseestimator} to obtain the following corollary for the standard probit model in \fref{eq:probitmodel}.
%
\begin{cor} \label{cor:lmmseestimator}
%
The L-MMSE estimate for the standard probit model in \fref{eq:probitmodel} is $\hat\bmx^\text{\em L-MMSE} = \bE^T \bC_\bmy^{-1}\bmy$,
where 
\begin{align*}
\bE & = \textstyle \left(\frac{2}{\pi}\right)^{1/2} \mathrm{diag}(\mathrm{diag}(\bC_\bmz)^{-1/2})\bD\bC_\bmx, \\
\bC_\bmy &= \textstyle \frac{2}{\pi} \arcsin ( \mathrm{diag}(\mathrm{diag}(\bC_\bmz)^{-1/2}) \bC_\bmz \\
& \quad \, \times \mathrm{diag}(\mathrm{diag}(\bC_\bmz)^{-1/2})),
\end{align*}
and $\bC_\bmz=\bD\bC_\bmx\bD^T+\bC_\bmw$. The associated MSE is given by $\textit{MSE}(\hat\bmx^\text{\em L-MMSE}) = \tr(\bC_\bmx - \bE^T \bC_\bmy^{-1} \bE)$.
%
\end{cor}


\subsection{Least Squares (LS) Estimator}
%
The L-MMSE estimator as in \fref{eq:LMMSE}  requires the computation of~$\bC_\bmy$ followed by a matrix inversion. For large-scale problems, one can avoid the matrix inversion by first solving $\bmy=\bC_\bmy \bmq$  for $\bmq$ using conjugate gradients \cite{wrightbook}, followed by calculating $\hat\bmx^\text{L-MMSE} = \bE^T\bmq$.  Hence, the complexity of L-MMSE estimation is comparable to that of MAP estimation. 
%
Computation of $\bC_\bmy$, however, cannot be avoided entirely. 
There exists a simpler linear estimator that avoids $\bC_\bmy$ altogether, which we call the least-squares (LS) estimator.
%
Concretely, let $M\geq N$ and consider the linearization in  \fref{eq:bussgang}, which is 
%\begin{align*} 
$\bmy=f_\sigma(\bmz)= \bE \bC^{-1}_\bmx\bmx+\bme$.
%\end{align*}  
By ignoring the residual error vector $\bme$ and by assuming that the columns of $\bE$ are linearly independent, we can simply invert the matrix $\bE \bC^{-1}_\bmx$, which yields the LS estimate
\begin{align} \label{eq:LSestimate}
\hat\bmx^\text{LS} = \bC_\bmx \bE^+\bmy
\end{align}
where $\bE^+=(\bE^T\bE)^{-1}\bE^T$ is the left pseudo-inverse of $\bE$. Again, one can use conjugate gradients to implement \fref{eq:LSestimate}.
%
In contrast to the L-MMSE estimator, the LS estimator does not require knowledge of $\bC_\bmy$, which makes it more efficient yet slightly less accurate (see the experimental results section for a comparison). 
%
As for the L-MMSE estimator, we have a closed-form expression for the MSE of the LS estimator.  
%
\begin{lem}  \label{lem:mseoflsestimator}
Assume that $\bE^+$ exists. Then, the MSE of the LS estimator in \fref{eq:LSestimate} is given by
\begin{align*}
\textit{MSE}(\hat\bmx^\text{\em LS}) = \tr(\bC_\bmx \bE^+\bC_\bmy(\bE^+)^T\bC_\bmx -\bC_\bmx).
\end{align*}
\end{lem}
%
\begin{proof}
The proof follows from the MSE definition \fref{eq:MSE}, and the facts that  $\Ex{}{\bmy\bmx^T}=\bE$ and $\bE^+\bE=\bI$.
\end{proof}



